Synthesize Dexterous Nonprehensile Pregrasp for Ungraspable Objects

Daily objects embedded in a contextual environment are often ungraspable initially. Whether it is a book sandwiched by other books on a fully packed bookshelf or a piece of paper lying flat on the desk, a series of nonprehensile pregrasp maneuvers is required to manipulate the object into a graspable state. Humans are proficient at utilizing environmental contacts to achieve manipulation tasks that are otherwise impossible, but synthesizing such nonprehensile pregrasp behaviors is challenging to existing methods. We present a novel method that combines graph search, optimal control, and a learning-based objective function to synthesize physically realistic and diverse nonprehensile pre-grasp motions that leverage the external contacts. Since the ``graspability'' of an object in context with its surrounding is difficult to define, we utilize a dataset of dexterous grasps to learn a metric which implicitly takes into account the exposed surface of the object and the finger tip locations. Our method can efficiently discover hand and object trajectories that are certified to be physically feasible by the simulation and kinematically achievable by the dexterous hand. We evaluate our method on eight challenging scenarios where nonprehensile pre-grasps are required to succeed. We also show that our method can be applied to unseen objects different from those in the training dataset. Finally, we report quantitative analyses on generalization and robustness of our method, as well as an ablation study.

==> intro_old.tex <==
\section{Introduction}
Manipulating environmental objects with a dexterous multi-fingered hand is a key human ability. Synthesizing dexterous manipulation motion is crucial to producing human-like animations. In particular, humans are proficient in \textit{nonprehensile manipulation}, which is to manipulate while utilizing external contacts. As an example, consider the task of removing a book from a densely packed bookshelf. It is challenging to directly grasp the book when it is occluded by the other books around it. A human would pivot the book outwards with one finger by leveraging the contact with the bookshelf, then grasp the book once enough area is exposed (Figure ~\ref{fig:bookshelf_demo}). This contrasts with other forms of manipulation such as simple grasping and in hand manipulation, where external contact is irrelevant to the desired motion.

%Manipulating environmental objects with a dexterous multi-fingered hand is a key human ability. Generating dexterous manipulation motion is crucial to producing human-like animations. In particular, humans are proficient in \textit{nonprehensile manipulation}, which is to manipulate while utilizing external contacts to provide extra support to the object when the object is occluded. Consider an example of removing a book from a densely packed bookshelf, it is hard to directly grasp and manipulate the book when it is initially occluded by other books around it. It is natural for human to first pivot the book out with one finger then grasp the book when there is enough area for grasping.  This contrasts with other forms of manipulation such as grasping and in hand manipulation, which either assume the object is not occluded and graspable or assume the object has already been placed in robot's hand. Both grasping and in hand manipulation fall short when object is initially occluded by environment.
% Manipulate different objects with dexterous hand is an important motion for virtual characters to interact with surrounding environment like a human. While this topic has been a active research focus for decades, most of recent research either focus in synthesising motion for object in hand manipulation\cite{openai_inhand} or motion for realistically grasping different objects \cite{grasptta}. Such trend leads to a natural question -- are these motion enough for animating all human manipulation? In our everyday life, we are often facing the scenario that the object we want to manipulate is neither already held in hand nor is easy for grasping. For example, when human try to pick up a book from a fully packed bookshelf, the target book is heavily occluded by other books and the bookshelf itself. It is very intuitive for a human to first pull the book out with one finger by pivoting then grasp the book to freely move that book around as shown in Fig. \ref{fig:bookshelf_demo}. However, such motion can not be generated by simply combining in-hand manipulation and grasping. It requires the character to utilize external contact from the bookshelf to pivot the book. This type of manipulation skill is defined as nonprehensile manipulation \cite{nonprehensile} and is an essential step toward synthesis general manipulation motion with dexterous hand.

Despite its prevalence as a human skill, nonprehensile manipulation has been much less studied in literature compared to other forms of manipulation. This is mainly due to the larger search space when considering different contacts between the target object, the dexterous hand, and the environment. The complexity prevents applying traditional planning and trajectory optimization algorithms directly.

%This is majorly due to the much larger search space when considering different contact mode between the target object, the dexterous hand and all other objects in the environment. The fact that there could be infinitely many contact points between the object and its surrounding environment prohibit traditional planning and trajectory optimization algorithm from being directly applied to these problems. Moreover, external contacts from environment are usually passive. This makes it very hard to control the amount of force exerted on the object from external contacts. Research works\cite{wenxuan} from robotics use reinforcement learning to solve nonprehensile manipulation problem with simple parallel gripper. However, the complexity of dexterous human hand from both geometry and number of degree of freedoms make this problem extra challenging. It is desirable to have a method dedicate for nonprehensile manipulation on dexterous hand that could fill in the gap between grasping and in hand manipulation.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/bookshelf_demo.jpeg}
  \caption{Pickup a book from bookshelf via nonprehensile manipulation}
  \label{fig:bookshelf_demo}
\end{figure}
\aw{Add some discussion on ``pregrasp'' in particular since that's what you are mostly doing.}

\aw{The text should be revised. I don't think it's very clear. It's also on the long side.} In this paper, we propose a multi-stage method for synthesising general nonprehensile manipulation motion for a biomimetic dexterous hand. We formulate the nonprehensile manipulation problem as a trajectory optimization problem in a object-centred formulation. Utilising an off-the-shelf stochastic trajectory optimizer such as MPPI\cite{mppi}, the trajectory optimization problem can be solved efficiently with over 90\% success rate. To avoid manually defining cost function for nonprehensile manipulation, we use a learned score function aims to expose the different objects for grasping and later in hand manipulation. We construct different scenarios that requires nonprehensile manipulation and demonstrate our method could work with different even unseen objects. We further compare our method against other method which didn't consider nonprehensile manipulation such as ManipNet\cite{manipnet}. Motion synthesised by our method is consistently more physically plausible and in general have higher motion quality than all other baselines. In summary our contributions are:

\begin{itemize}
    \item A general pipeline for synthesizing nonprehensile pregrasp motion.
    \item A trajectory optimization formulation for non-prehensile manipulation with contact that can be efficiently solved using MPPI.
    \item A learned objective function for solving realistic general nonprehensile pregrasp problem.
\end{itemize}

% Add a bullet point version







==> notes.tex <==
Evaluation
Settings
- Quality and diversity of results: Overview of all results; same object in diverse environments 
- Generalizibility of learning components to other objects and other scenarios: All examples are different from training data. In addition, we change the scales of the objects systematically
- Robustness of algorithms: Easy to discover a successful path; the successful paths are robust
- Compare with ManipNet
- Ablation on Score function design


\section{Evaluation}
We evaluate our method qualitatively by demonstrating a rich and diverse set of synthesized hand animations, as well as quantitatively by reporting experimental results on robustness, generalizability, algorithm design, and comparisons with the most relevant existing method. We use a Shadow Hand model with $28$ DoFs ($22$ joint and $6$ base DoFs) in our implementation, but the proposed method is agnostic to the choice of hand model. We use PyBullet\cite{pybullet} physics simulator and SNOPT nonlinear optimization solver \cite{SNOPT} for trajectory optimization. Inverse kinematics problems are soled using the Collision-free IK Module in Drake\cite{drake}.

\subsection{Motion quality and diversity}
We design eight diverse scenarios to test our method, including adjacent books on a bookshelf, a ruler lying flat near the edge of a table, a computer keyboard and a flat cardboard placed on a shelf against a wall, a dining plate and a lunch box placed in the middle of the table, a densely packed spice rack, and a marker stored in a pencil box. We show that our method is able to synthesize natural and physically plausible non-prehensile pregrasp to move the objects into a graspable configuration for all various scenarios. Figure \ref{fig:tasks} and the supplemental video show the keyframes and animations of our results.

To further demonstrate the diversity of motions generated by our method, we showcase a few scenarios in which multiple successful pregrasp strategies exist. By simply searching more paths on the contact graph instead of exiting upon the first successful path, our method is able to generate visually and functionally different animations. Figure \ref{fig:diverse} (a) and (b) show two different ways to pick up the cardboard: one uses the index finger to pull the cardboard outward while the other one uses the thumb. Changing the surrounding of the object can also result in different pregrasp strategies. If the keyboard is placed near the backboard of the shelf, the hand would push the keyboard against the backboard to pivot it up (Figure \ref{fig:diverse} (c)). If the keyboard is placed near the edge of the shelf, the hand would lift the keyboard from the corner that has been fully exposed \karen{Double check.}.

\subsection{Robustness of algorithms}
We define two metrics to evaluate the robustness of our method.
\paragraph{Grasp success rate.}
Feasibility of the grasp generated by the grasp generator is the most critical indicator of the success of our method. A feasible grasp must satisfy both dynamics and kinematics constraints (Section XXX). Since we use a sampling-based grasp generator (i.e. a CVAE), we compute the success rate of the grasp as $r_\text{suc}=\frac{\# \text{feasible}\;\text{grasps}}{\# \text{latent}\;\text{space}\; \text{samples}}$. We set number of latent space samples to be $20$ in our experiments.

\paragraph{Number of paths attempted.} The sampling-based optimizer might need to sample a number of candidate contact paths before a feasible one is found. The number of paths attempted is another metric to measure efficiency of our algorithm. For each optimized path, we test a set of $20$ grasps generated by different latent space samples of the grasp generator. If there exists one feasible grasp, the path is considered successful and the number of paths attempted thus far is reported as $N_\text{paths}$.

We evaluate $r_\text{suc}$ and $N_\text{paths}$ on all eight scenarios shown in Figure \ref{fig:tasks}. The results show that...

\subsection{Generalization to unseen objects}
Since our method contains learning-based components trained on a dataset of objects, it is crucial to demonstrate the generalizability of the method on unseen objects. All eight scenarios we described above use unseen objects different from the YCB training dataset. In addition, we evaluate the method on a few nonconvex objects. For those objects that can be reasonably approximated by their convex hulls, such as a tape roll and a cookie jar (Figure \ref{fig:taperoll}), our method can successfully synthesize plausible motions. However, for highly non-convex objects, our current implementation is limited by the mesh reconstruction algorithm which assumes convexity and the Drake IK solver which only supports collision avoidance for convex geometry. More failure cases and limitations can be found in the supplemental video. \karen{Is the above text on convex limitation true?}

We also systematically evaluate the generalizability on the scales of geometry using the metrics $r_\text{suc}$ and $N_\text{paths}$. Table \ref{tab:scale} shows that... 

\subsection{Ablation on Score Function Design}

We perform an ablation study on the design choice of the score function. We evaluate two variants of the score function: 1) No SDF: only use positions of the points on the object surface as input to the point cloud encoder; 2) No Shape: only use signed distance values as input to the point cloud encoder. We compute $r_\text{suc}$ and $N_\text{paths}$ on these two variants using the plate and the marker examples. \ref{tab:ablation} shows that having both SDF and object shape information is crucial for accurately assessing the score of a grasp.

\subsection{Comparison with ManipNet}
Due to the lack of existing methods on non-prehensile manipulation for dexterous hand, we compare our method with the state-of-the-art kinematics method ManipNet \cite{manipnet} on the spice rack example. We pick this example because ManipNet has been trained on grasping objects with similar cylinder shapes. \ref{fig:compare_manipnet} shows that, despite the ability to sense the environment, ManipNet attempts to grasp the bottle without considering the surrounding objects, resulting in severe finger penetration. In contrast, our method is able to first pull out the bottle and then grasp without colliding with other objects. We acknowledge that the comparison would have been more fair if ManipNet has been trained with similar surrounding objects. However, recording training data that covers the space of possible surroundings for all different objects is impractical and makes the approach of ManipNet difficult to extend to contextual environments.





\section{Introduction}
Manipulating objects with a dexterous multi-fingered hand is a key human ability. In particular, humans are proficient at leveraging environmental contacts to perform tasks that are otherwise impossible, utilizing \textit{nonprehensile manipulation}, a strategy to move objects without establishing a firm grasp first.  For instance, when removing a book from a densely packed bookshelf, one would pivot the book outwards with one finger while keeping the book stabilized with lateral environment contacts. Once sufficient area of the book is exposed, the book can be picked up with a simple grasp (Figure ~\ref{fig:teaser}). This type of non-prehensile ``pregrasps'' is essential for operating in an ecological human living space in which objects are often initially ungraspable due to occlusion by other surrounding objects.

Replicating human-like nonprehensile manipulation is challenging to existing motion planning methods. The inclusion of environmental contacts leads to combinatorial complexity in the number of possible contact configurations, which is intractable to even the state-of-the-art motion planners. Moreover, it is difficult to define heuristics for the purpose of trajectory optimization. Consequently, many papers in both the dexterous grasp generation literature (e.g.,~\cite{grasptta, graspfield, grabnet}) and the motion generation literature (e.g.,~\cite{manipnet}) involve motion generation through learning-based method. Nevertheless, the rich contact constraints in manipulation makes it difficult for learning method to produce physically realistic motions with no interpenetrating or telekinetic interactions. The tradeoff between computational efficiency and physical realism remains a major hurdle in synthesizing manipulation motion.

%\eric{most related to this statement is \cite{manipnet}, however grasp generation frame work such as \cite{grasptta, graspfield, grabnet} can also be used as an example. Another related branch is hand pose estimation given object pose and some rough motion data from hand such as \cite{handestimation}}.

In this paper, we propose a method to efficiently synthesize physically realistic, non-prehensile grasping, utilizing surrounding objects in cluttered environments. We focus on generating pregrasp motions that move ungraspable objects to graspable poses using environmental contacts. Our key observation is that, for any object placed in the environment, \emph{at most two} finger contacts are necessary for non-prehensile pregrasp since there exist at least one external contact point which collectively achieves wrench closure with the two finger contacts. This significantly reduces the search space of our motion synthesis problem, and allows us to formulate pregrasp planning as a reasonably sized mixed-integer optimization problem. Under this observation, our method solves for at most two sequences of contact points on the object by formulating a combination of discrete graph search and trajectory optimization.

However, defining an exact metric to measure “graspability” during the pregrasp phase is not trivial. The obvious goal in this phase is to expose the surface of the object, but it has to be done in such a way that the finger contacts during the pregrasp phase can be fluidly transitioned to a firm grasp later. As such, the graspability we would like to maximize depends on the current state of the object, the environment, the fingers that have established contact points and the fingers that are still free of contact. To avoid relying on heuristics and to be able to gereanlize to different scenarios, we use a learning approach to learn a general metric of “graspability” through a dataset of dexterous grasps in various scenarios. Using this metric, we perform particle-based trajectory optimization in a physics-based simulator. This allows \aw{todo}

able to produce trajectories certified to be physically feasible by the simulation.\aw{todo}

We demonstrate our method on 8 challenging scenarios where nonprehensile manipulation is required to successfully grasp the object. Our method significantly outperformed \aw{... todo.}



\subsection{Trajectory optimization}
The second stage searches for optimal trajectories for the two finger tips and the object that lead to a force-closure grasp using 3-5 fingers. The optimization process involves a double-loop iteration. The outer loop solves a discrete path planning problem while the inner loop solves a continuous dynamic optimization. 

A path consists of $N$ nodes connected by edges on $\mathcal{G}$. Since the initial object state is in the context of $\mathcal{O}$, we restrict the first node of each path to be a node in $\mathcal{V}_c$. The remaining $N-1$ nodes can be any node on $\mathcal{C}$. We compute the score of all possible paths and sort the paths by their score from high to low:
\begin{equation}
s_{path} = s_c(\bm{v}_1) + \sum_{i=2}^{N} s_n(\bm{v}_i),
\end{equation}
where $s_c$ and $s_n$ are overloaded to indicate functions that return the score of an input node.

The outer loop of the optimization iterates over the sorted list of paths until a successful trajectory is found by the inner loop. For each given path $\mathcal{P} = (\bm{v}_1, \cdots, \bm{v}_{N})$, the inner loop solves for the contact locations of the finger tips within the boundary of the triangles associated with the nodes in the $\mathcal{P}$. Formally, we optimize the state variable $\bm{x}_t = (\bm{p}^1_t, \bm{p}^2_t, b_t)$, where $t = 1 \cdots N$, and the control variables $\bm{u} = (\bar{\bm{p}}^1_t, \bar{\bm{p}}^2_t)$, where $t=K \cdot N$. $\bm{p}^1_t$ and $\bm{p}^2_t$ are the thumb position and the index finger position in the object coordinate frame at the contact stage $t$. $b_t$ is a discrete variable that indicates whether the contact state is thumb-only, index-finger-only, or both-fingers at contact stage $t$. The control variables, $(\bar{\bm{p}}^1_t, \bar{\bm{p}}^2_t)$, define the target locations of the thumb and the index finger in the world coordinate frame at frame $t$, respectively. Because the contact forces tend to change in a higher resolution than the contact locations, we allow the control variables to change $K$ times within each contact stage. The objective function for the optimization is defined as follows:
\begin{equation}
\sum_{t=i}^N\; f_\theta\big((b_t!=\mathrm{index-only})?\bm{p}^1_t:\empthset , (b_t!=\mathrm{thumb-only})?\bm{p}^2_t:\empthset, \mathcal{O}_t\big), 
\end{equation}
where $\mathcal{O}_t$ depends on the object state, essentially a function of $\bm{x}_{1:t}$ and $\bm{u}_{1:t}$ via physics simulation. To ensure the contact locations staying within the boundary of the given triangles, we use the baricentric coordinates to parameterize $\bm{p}^1$ and $\bm{p}^2$. 

To further ensure physical plausibility of the finger motion, a finger can only change the location after it is detached from the object in the previous contact stage. For example, $b_{t-1}$ must be "thumb-only" for the index finger to change the location at $t$. This additional constraint prevents fingers from instantaneously jump from one location to another.

We use a sample-based optimizer, MPPI\cite{MPPI}, since gradient based optimization algorithms tend to stuck in local minima when solving contact-rich control tasks \cite{bundlegradient}. 

After solving each trajectory optimization problem, we query the grasp generator, $\g_\phi$ to predict a grasp based on the terminal object state and the locations of thumb and the index finger tips. If a predicted grasp is feasible, we stop searching other paths. 

-----------



At the start of each trajectory optimization, the path with highest score is selected. We search from the highest scored path until a feasible grasp could be found after running trajectory optimization. Given a path on contact state graph from previous stage, we solve a trajectory optimization problem whose contact points is constrained by the nodes on the path. Formulating and solving a trajectory optimization problem to enable non-prehensile manipulation is challenging. On the one hand, the discontinuous nature of the problem makes solving the problem by brute force via off-the-shelf solver extremely difficult. On the other hand, it is hard to define a general cost function that are suitable for all scenarios requiring non-prehensile manipulation. 
\paragraph{Problem formulation}
To address the first issue, we took an object-centred approach to formulate the trajectory optimization problem hierarchically at different time scale. Formally, at each time step, our decision variables for a fingertip i are: $\mathbf{a}_i(t)=[\mathbf{p}^o_1(t), \mathbf{p}^o_2(t), \tilde{\mathbf{p}}^w_i(t), b_i(t)]$, where $\mathbf{p}^o_1, \mathbf{p}^o_2$ are the thumb and index finger tip position on the object surface expressed in patch local coordinate, notice that $\mathbf{p}^o_1, \mathbf{p}^o_2$ cannot go beyond the boundaries of the patches specified by the node $v$ in contact state graph. For instance, if the patch is a triangle and the patch local coordinate is barycentric coordinate $[\alpha, \beta]$, then $\alpha\ge 0, \beta\ge 0$ and $\alpha+\beta\le 1$ must be satisfied. $ \tilde{\mathbf{p}}^w_i(t)$ is target position of that fingertip in world coordinate. $b(t)$ is a binary decision variable which determine whether the fingertip is in contact with the object or not. Notice that different decision variables are changing at different frequency, when solving trajectory optimization problem only $\tilde{\mathbf{p}}^w_i(t)$ is changing at every time step, while $\mathbf{p}^o_t$ and $b(t)$ are changing every K steps. We also move one node forward in contact state graph every K steps. This design is based on the observation that when human manipulate an object, finger gait is not always changing instantaneously. To further ensure the naturalness of finger motion, constraint is set that the tip contact position $\mathbf{p}^o_i$ is only allow to change after fingertip is detached from the object in the previous step ($b_i$ is set to 0). This prevent fingertip from teleportation from one position to another and improve the physical plausibility of the motion. Fig. \ref{fig:action} shows how decision variables are set across different time steps. Another design which allow us to solve the trajectory optimization problem efficiently is that we only consider at most two fingertips during non-prehensile manipulation phase. Since during non-prehensile manipulation, at least one external contact point is utilised to manipulate the object, we only need at most 2 extra contact point provided by the fingertips to achieve force and torque closure. 

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/action.png}
  \caption{Illustration of how decision variables are set. From t=0 to t=10, $b_i=1$, from t=10 to t=20 $b_i=0$ and from t=20 onward, $b_i=1$}
  \label{fig:action}
\end{figure}

As for the cost function of the optimization problem, we use a learned score function $f_\theta(\mathbf{s}_\text{obj},\mathbf{s}_\text{finger})$ to evaluate how good current state is for a successful grasp. Here $\mathbf{s}_\text{obj}$ contains object's pointcloud and signed distance function value at each point , $\mathbf{s}_\text{finger}$ is position of fingertips in object-centred frame and $\theta$ is learnable parameters inside neural network. In general, we hope to manipulate the object to expose a graspable pose during non-prehensile manipulation phase. More details on score function design and training will be described in \ref{subsec:scorefunction, subsec:dataset}

\paragraph{Optimization algorithm} % Should be merged in to previous one
After a contact state graph is constructed, we rank all possible paths on that graph by cumulative score of each node. We start searching for a feasible trajectory from the path with highest score and use it to solve trajectory optimization problem. We use MPPI\cite{MPPI} to optimize the trajectory as gradient based optimization algorithm tend to stuck in local minima in contact-rich control task\cite{bundlegradient}. After solving each trajectory optimization problem, we query a grasp generator to predict a grasp based on the terminate object pose and fingertip placement. If a predicted grasp is feasible, we stop searching other paths. 






\subsection{Build contact state graph}
Given an object mesh $\mathcal{M}$ and the SDF to the environment $\mathcal{O}$, we construct a contact state graph $\mathcal{G}$ such that rich hand-object contact behaviors to be feasibly explored by an optimization process (Section XXX). To construct $\mathcal{G}$, we simplify $\mathcal{M}$ to XXX triangles via an off-the-shelf mesh simplification algorithm \cite{XXX} (Figure \ref{fig:contactstate}). Since we only consider the thumb and the index finger making contact with the object, we define each node in the graph as $\bm{v} = (\mathcal{T}_1, \mathcal{T}_2)$, where $\mathcal{T}_1$ and $\mathcal{T}_2$ indicate the triangles that the thumb and the index finger are in contact with, respectively. Because many of the triangle pairs are not ideal contact locations for non-prehensile pregrasp, we use the learned score function $f_\theta$ to prune the nodes and only keep the high-scoring nodes in $\mathcal{G}$. 

For each node $\bm{v}$, we compute two scores, $s_c$ and $s_n$, to consider the feasibility of the node within the context of the environment and without:
\begin{equation}
s_c = f_\theta(\bm{p}_1, \bm{p}_2, \mathcal{O}); \;\;\;\; s_n = f_\theta(\bm{p}_1, \bm{p}_2, \empty).
\end{equation}
We sample five finger tip locations within $\mathcal{T}_1$ and $\mathcal{T}_2$ associated with $\bm{v}$ for each of the three scenarios: thumb-only contact, index-finger-only contact, and two-finger contact. We query $f_\theta$ for these 15 finger tip placements and compute the average $s_c$ and $s_n$ for $\bm{v}$. If either $s_c$ or $s_n$ are within the top $M$ percentile, we include $\bm{v}$ in $\mathcal{G}$. If $v$ is selected due to a high $s_c$, we put it in a subset call $\mathcal{V}_c$. This subset of nodes will be used for the initial contact state in the optimization process (Section XXX). 

The nodes must be connected by edges to indicate feasible contact state transitions.
To prevent two fingers simultaneously changing contact locations, we only connect two nodes by an edge if they share the same triangle for the thumb or for index finger. Each node also connects to itself to allow for consecutive unchanged contact states (Figure XXX). 
